Learning Multi-item Auctions with (or without) Samples

We provide algorithms that learn simple auctions whose revenue is approximately optimal in multi-item multi-bidder settings, for a wide range of valuations including unit-demand, additive, constrained additive, XOS, and subadditive. We obtain our learning results in two settings. The first is the commonly studied setting where sample access to the bidders' distributions over valuations is given, for both regular distributions and arbitrary distributions with bounded support. Our algorithms require polynomially many samples in the number of items and bidders. The second is a more general max-min learning setting that we introduce, where we are given "approximate distributions," and we seek to compute an auction whose revenue is approximately optimal simultaneously for all "true distributions" that are close to the given ones. These results are more general in that they imply the sample-based results, and are also applicable in settings where we have no sample access to the underlying distributions but have estimated them indirectly via market research or by observation of previously run, potentially non-truthful auctions. Our results hold for valuation distributions satisfying the standard (and necessary) independence-across-items property. They also generalize and improve upon recent works, which have provided algorithms that learn approximately optimal auctions in more restricted settings with additive, subadditive and unit-demand valuations using sample access to distributions. We generalize these results to the complete unit-demand, additive, and XOS setting, to i.i.d. subadditive bidders, and to the max-min setting. Our results are enabled by new uniform convergence bounds for hypotheses classes under product measures. Our bounds result in exponential savings in sample complexity compared to bounds derived by bounding the VC dimension, and are of independent interest.

==> iid_XOS.tex <==
\notshow{ 
\subsection{i.i.d. Buyers}
%For the SPM, when buyers are i.i.d. and regular, the supply limiting mechanism (by Tim, Inbal and Qiqi) achieves a constant fraction of its revenue and only requires $1$ sample. Need to figure out what to do when the distributions are bounded between $[0,1]$ or we only have $\hat{D}$.
In this section, we consider the case where bidders are symmetric, i.e., $D_{i}=D_{k}$ for any bidder $i$ and $k$. We simply use $D_j$ to denote the type distribution for item $j$, and we let $\DD =\times_{j} D_j$.


\begin{theorem}\cite{CaiZ17}
	For symmetric bidders, the better of an RSPM and the following ASPE achieves at least $\frac{1}{C}$ fraction of the optimal revenue for some absolute $C\geq 1$. Suppose $\{\beta_j\}_{j\in[m]}$ is a collection of real numbers such that $F_j(\beta_j)\in[1-\frac{1}{2n},1-\frac{1}{4n}]$ for all $j\in[m]$. If  $\sum_j F_j\left(\beta_j+c\right) \geq \frac{2}{3}$, let $c= 0$. Otherwise, let $c$ be a nonnegative real number such that $\sum_j F_j\left(\beta_j+c\right) \in [\frac{1}{2}, \frac{2}{3}]$.
\end{theorem}
For the anonymous sequential posted price with entry fee mechanism, we need to estimate the price $p_j$ for each item $j$, which requires the following statistics. Here let $t_i$ be the type of bidder $i$ and $v(t_i,S)$ be bidder $i$'s value for winning set $S$. In particular, let $V_{j}(t_i)$ be the value for winning just item $j$.
\begin{itemize}
\item $\beta_j := \Pr_{t\sim D}[V_j(t)\geq \beta_j]=1/2n$.
\item If $m>n$, $c:= \sum_j \Pr_{t\sim D}[V_j(t)\geq \beta_j+c]=1/2$, otherwise $c:=0$.
\item Let $C_i(t_i):=\{j\ |\ V_j(t_i)<\beta_j+c\}$.
\item Let $$p_j = \sum_i\sum_{t_i}f(t_i)\cdot \sum_{S:j\in S} \sigma_{iS}(t_i) \gamma_{j}^{S}(t_i),$$ where $\sigma_{iS}(t_i)$ is the interim probability for buyer $i$ to receive bundle $S$. Let $v_{j}^{(S)}(t_i)$ be the supporting price of item $j$ for set $S$ if the bidder's type is $t_i$ \footnote{$v_{j}^{(S)}(t_i)=t_{ij}$ when $t_i$ is additive subject to some constraints, but when $v_i$ is XOS the supporting prices depends on which bundle buyer $i$ is receiving.}, then $\gamma_{ij}^{(S)}(t_i)=v_{j}^{(S\cap C_i(t_i))}$ if $j\in S\cap C_i(t_i)$, and $\gamma_{ij}^{(S)}(t_i)=0$ otherwise.
\end{itemize}

What I can prove is that for any allocation rule $\sigma$, if we set the correct entry fee, then the anonymous posted price mechanism with entry fee has revenue at least $\frac{1}{2}\cdot \sum_j p_j$. Clearly, we need should use the $\sigma$ that maximizes $\sum_j p_j$.

Let $v'(t_i,S) = v(t_i, S\cap C_i(t_i))$ and $\sum_j p_j$ is the same as the social welfare for allocation $\sigma$ when $v'(\cdot,\cdot)$ is the valuation function. Clearly, $\sum_j p_j$ is maximized when we take $\sigma$ to be the welfare maximizing allocation for $v'(\cdot,\cdot)$.


I think as long as we can estimate all the $p_j$ within error $\delta$, we will lose revenue at most $O(m\delta)$. Of course, this will also require us to estimate $\beta_j$ and $c$. %For valuations that are additive subject to downwards closed constraints, it is easy to estimate $p_j$. As for any $S$,  $\bar{v}^{(S)}_{ij}=\bar{v}_{ij}=v_{ij}\cdot \ind[v_{ij}\leq \beta_j+c]$, so we only need to take $\sigma$ as the VCG allocation rule for $\bar{v}_{ij}$. But for XOS valuations, since the supporting prices depend on $S$, it is unclear what is the optimal $\sigma$.
}


==> subadditive_local.tex <==
\section{Symmetric Bidders}\label{sec:symmetric bidders}
Finally, we consider symmetric bidders ($D_i=D_{i'}$ for all $i$ and $i'\in[n]$). We only describe the results here and postpone the formal statements and proofs to Appendix~\ref{sec:symmetric appx}.
 \begin{itemize}
 	\item  \textbf{XOS valuations:} we can learn in polynomial time an approximately optimal mechanism with a polynomial number of samples when the valuations are XOS over independent items. \yangnote{Our algorithm essentially estimates all the parameters needed to run the RSPM and ASPE used in~\cite{CaiZ17}. In general, it is not clear how to estimate these parameters efficiently. But when the bidders are symmetric, one only needs to consider ``symmetric parameters'' which greatly simplifies the search space and allows us to estimate all the parameters in polynomial time. }See Appendix~\ref{sec:symmetric XOS} for details.
 	\item \textbf{subadditive valuations:} when the valuations are subadditive over independent items,  the optimal revenue is at most $O\left(\frac{n}{\max\{m,n\}}\right)$ times larger than the highest revenue obtainable by an RSPM. In other words, if the number of items is within a constant times the number of bidders, an RSPM suffices to extract a constant fraction of the optimal revenue.  Applying our results for unit-demand bidders in Section~\ref{sec:unit-demand}, we can learn a nearly-optimal RSPM, which is also a good approximation to $\opt$. In fact, when the distribution for random variable $V_i(t_{ij})$ is regular for every bidder $i$ and item $j$, we can design a prior-independent mechanism\footnote{In other words, our mechanism does not take any sample from $D$.} that achieves a constant fraction of the optimal revenue. See Appendix~\ref{sec:symmetric subadditive} for details.
 \end{itemize}



==> unit-demand_old.tex <==
\section{Unit-demand Valuations} \label{sec:unit-demand}

In this section, we show how to learn approximately revenue-optimal mechanisms for unit-demand valuations. It is known that there always exists a sequential posted price mechanism (SPM) that achieves at least $\frac{1}{24}$ of the optimal revenue~\cite{ChawlaHMS10, KleinbergW12, CaiDW16}. Our plan is to show that under all three models, we can learn a good sequential posted price mechanism that approximates the optimal revenue well.

\begin{algorithm}[ht]
\begin{algorithmic}[1]
\REQUIRE $P_{ij}$ is the price for bidder $i$ to purchase item $j$.
\STATE $S\gets [m]$
\FOR{$i \in [n]$}
	\STATE Show bidder $i$ {the} set of available items $S$.
	 \STATE $i$ purchases her favorite bundle $S_i^{*}\in \max_{S'\subseteq S} v_i(t_i, S') - \sum_{j\in S'} P_{ij}$ and pays $\sum_{j\in S_i^{*}}P_{ij}$.
        \STATE $S\gets S\backslash S_i^{*}$.
\ENDFOR
\end{algorithmic}
\caption{{\sf Sequential Posted Price Mechanism (SPM)}}
\label{alg:seq-mech}
\end{algorithm} 

\subsection{Unit-demand Valuation: direct access to approximate distributions}\label{sec:unit-demand Kolmogorov}
We first consider the model where we only have access to an approximate distribution $\hat{D}$. The following definition is crucial for proving our result. 

\begin{definition}
For any single dimensional distribution $\DD$ with cdf $F$, we define its revenue curve $R_{\DD}: [0,1]\mapsto \mathbb{R}_{\geq 0}$ as
	\begin{align*}
	{R}_{\DD} (q) = &\max  x\cdot \ubar{q}\cdot {F}^{-1}(1-\ubar{q}) +(1-x)\cdot \bar{q}\cdot {F}^{-1}(1-\bar{q})\\
	& \qquad\textbf{s.t. } x\cdot \ubar{q}+(1-x)\cdot \bar{q}=q\\
	&  \qquad\qquad x, \ubar{q}, \bar{q} \in [0,1]
\end{align*}
where $F^{-1}(1-p) = \sup\{x\in R: \Pr_{v\sim \DD}[v\geq x]\geq p\}$.
\end{definition}


% For any bidder $i$ and item $j$, define function $R_{\hat{D}_{ij}}: [0,1]\rightarrow \mathbb{R}_{\geq 0}$ as:
%We define $R_{\hat{D}_{ij}}$ similarly with respect to $\hat{F}_{ij}$.
%It is not hard to argue that $R_{\hat{D}_{ij}}(\cdot)$ is exactly the ironed revenue curve for distribution $\hat{D}_{ij}$.

\begin{lemma}
	Let ${\varphi}_{ij}(\cdot)$ and $\hat{\varphi}_{ij}(\cdot)$ be the ironed virtual value function for distribution $D_{ij}$ and $\hat{D}_{ij}$ respectively, then for any $q\in [0,1]$, ${R}_{D_{ij}}(q) = \int_{{F}^{-1}_{ij}(1-q)}^H {\varphi}(x) dF(x)$ and $R_{\hat{D}_{ij}}(q) = \int_{\hat{F}^{-1}_{ij}(1-q)}^H \hat{\varphi}(x) dF(x)$. Since the ironed virtual value function is monotonically non-decreasing, ${R}_{D_{ij}}(\cdot)$ and $R_{\hat{D}_{ij}}(\cdot)$ are concave functions. 
\end{lemma}
\yangnote{Fill in the proof later.}

Next, we provide an upper bound of the optimal revenue using $R_{D_{ij}}$.
\begin{lemma}\label{lem:UB for UD rev}
For unit-demand bidders, there exists a collection of non-negative numbers $\{q_{ij}\}_{i\in[n], j\in[m]}$ satisfying $\sum_i q_{ij}\leq 1$ for all $j\in [m]$ and $\sum_j q_{ij}\leq 1$ for all $i\in [n]$, such that the optimal revenue $$\opt\leq 4\cdot \sum_{i,j} R_{D_{ij}}(q_{ij}).$$
\end{lemma}
\begin{proof}
As shown in~\cite{CaiDW16}, $\opt\leq 4 \copies$. Let $q_{ij}$ be the ex-ante probability that agent $(i,j)$ is served in the optimal mechanism for the copies setting. Chawla et al.~\cite{ChawlaHMS10} showed that $\copies\leq \sum_{i,j} R_{D_{ij}}(q_{ij})$. Our statement follows from the two inequalities above.\end{proof}

Next, we consider a convex program (Figure~\ref{fig:CP unit demand}) and argue that the value of the optimal solution of this program is at least $\frac{1}{8}$ of the optimal revenue.
\begin{figure}[ht]
%\colorbox{MyGray}{
\begin{minipage}{\textwidth} 
\begin{align*}\label{prog:convex ud}
&\max \sum_{i,j} R_{D_{ij}}(q_{ij})\\
\textbf{s.t. }& \sum_i q_{ij}\leq \frac{1}{2}\qquad \text{ for all $j\in[m]$}\\
& \sum_j q_{ij}\leq \frac{1}{2}\qquad \text{ for all $i\in[n]$}\\
& q_{ij}\geq 0\qquad \text{ for all $i\in[n]$ and $j\in[m]$}
\end{align*}
\end{minipage}
\caption{A Convex Program for Unit-demand Bidders with Exact Distributions.}
\label{fig:CP unit demand}
\end{figure}

\begin{lemma}\label{lem:compare exact CP with opt}
	The optimal solution of convex program in Figure~\ref{fig:CP unit demand} is at least $\frac{\opt}{8}$.
\end{lemma}
\begin{proof}
	Let $\{q'_{ij}\}$ be the collection of nonnegative numbers in Lemma~\ref{lem:UB for UD rev}. Clearly, $\left\{\frac{q_{ij}'}{2}\right\}$ is a set of feasible solution for the convex program. Since $R_{D_{ij}}(\cdot)$ is concave, $R_{D_{ij}}\left(\frac{q_{ij}'}{2}\right)\geq \frac{R_{D_{ij}}(q'_{ij})}{2} + \frac{R_{D_{ij}}(0)}{2}=\frac{R_{D_{ij}}(q'_{ij})}{2}$. Therefore, $$\sum_{i,j} R_{D_{ij}}\left(\frac{q_{ij}'}{2}\right)\geq 
	\frac{1}{2}\cdot \sum_{i,j} R_{D_{ij}}(q'_{ij})\geq \frac{\opt}{8}.$$
\end{proof}

If we know all $F_{ij}$ exactly, we can solve the convex program (Figure~\ref{fig:CP unit demand}) and use the optimal solution to construct an SPM via an approach provided in~\cite{ChawlaHMS10,CaiDW16}. The constructed sequential posted mechanism has revenue at least $\frac{1}{4}$ of the optimal value of the convex program, which is at least $\frac{\opt}{32}$. Next, we show that with only access to $\hat{F}_{ij}$, we can essentially carry out the same approach. Consider a different convex program (Figure~\ref{fig:CP unit demand approximate dist}).
\begin{figure}[ht]
\begin{minipage}{\textwidth} 
\begin{align*}
&\max \sum_{i,j} R_{\hat{D}_{ij}}(q_{ij})\\
\textbf{s.t. }& \sum_i q_{ij}\leq \frac{1}{2} + n\cdot\epsilon\qquad \text{ for all $j\in[m]$}\\
& \sum_j q_{ij}\leq \frac{1}{2}+m\cdot\epsilon \qquad \text{ for all $i\in[n]$}\\
& q_{ij}\geq 0\qquad \text{ for all $i\in[n]$ and $j\in[m]$}
\end{align*}
\end{minipage}
\caption{A Convex Program for Unit-demand Bidders with Approximate Distributions.}
\label{fig:CP unit demand approximate dist}
\end{figure}

In the following Lemma, we prove that the optimal values of the two convex programs above are close. \todo{If time permits, prove that if the support size for all $\hat{D}_{ij}$ is at most some finite number $s$, the convex program above can be rewritten as a linear program with size $\poly(n,m,s)$.}
\begin{lemma}\label{lem:UD compare the two CP}
	Let $\{{q}^*_{ij}\}_{i\in[n],j\in[m]}$ and $\{\hat{q}_{ij}\}_{i\in[n],j\in[m]}$ be the optimal solution of the convex program in Figure~\ref{fig:CP unit demand} and~\ref{fig:CP unit demand approximate dist} respectively.	$$\sum_{i,j}R_{\hat{D}_{ij}}(\hat{q}_{ij})\geq \sum_{i,j}{R}_{D_{ij}}({q}^*_{ij})-\epsilon\cdot mn H.$$
	\end{lemma}

\begin{proof}
	We first fix some notations. For any bidder $i$ and item $j$, let $\ubar{q}^*_{ij}, \bar{q}^*_{ij}$ and $x_{ij}$ $\in[0,1]$ be the numbers satisfy that $x_{ij}\cdot \ubar{q}^*_{ij}\cdot {F_{ij}}^{-1}(1-\ubar{q}^*_{ij}) +(1-x_{ij})\cdot \bar{q}^*_{ij}\cdot {F_{ij}}^{-1}(1-\bar{q}^*_{ij})=R_{D_{ij}}(q^*_{ij})$ and $x_{ij}\cdot \ubar{q}^*_{ij} +(1-x_{ij})\cdot \bar{q}^*_{ij}=q^*_{ij}$. Let $\ubar{p}_{ij} = {F_{ij}}^{-1}(1-\ubar{q}^*_{ij})$, $\bar{p}_{ij} = {F_{ij}}^{-1}(1-\bar{q}^*_{ij})$, and  $q'_{ij} = x_{ij}\cdot \left(1-\hat{F}_{ij}(\ubar{p}_{ij})\right)+(1-x_{ij})\cdot \left(1-\hat{F}_{ij}(\bar{p}_{ij})\right)$. By the definition of $R_{\hat{D}_{ij}}(\cdot)$, \begin{equation}\label{eq:compare revenue curve}
		R_{\hat{D}_{ij}}(q_{ij}')\geq x_{ij}\cdot \left(1-\hat{F}_{ij}(\ubar{p}_{ij})\right)\cdot \ubar{p}_{ij}+(1-x_{ij})\cdot \left(1-\hat{F}_{ij}(\bar{p}_{ij})\right)\cdot \bar{p}_{ij}
	\end{equation} Since $||\hat{D}_{ij}-D_{ij}||_K\leq \epsilon$, $\hat{F}_{ij}(\ubar{p}_{ij})\in [1-\ubar{q}^*_{ij}-\epsilon, 1-\ubar{q}^*_{ij}+\epsilon]$ and $\hat{F}_{ij}(\bar{p}_{ij}) \in [1-\bar{q}^*_{ij}-\epsilon, 1-\bar{q}^*_{ij}+\epsilon]$. Hence, the RHS of inequality~(\ref{eq:compare revenue curve}) is greater than $R_{D_{ij}}(q_{ij}^*)-\epsilon\cdot H$. Therefore, $R_{\hat{D}_{ij}}(q_{ij}')\geq R_{D_{ij}}(q_{ij}^*)-\epsilon\cdot H$.
	
	Next, we argue that $\{q'_{ij}\}_{i\in[n],j\in[m]}$ is a feasible solution for the convex program in Figure~\ref{fig:CP unit demand approximate dist}. Since $1-\hat{F}_{ij}(\ubar{p}_{ij})\leq \ubar{q}^*_{ij}+\epsilon$ and $1-\hat{F}_{ij}(\bar{p}_{ij})\leq \bar{q}^*_{ij}+\epsilon$, $q'_{ij}\leq q^*_{ij}+\epsilon$. Thus, $\sum_i q'_{ij} \leq \sum_i q^*_{ij} + n\cdot \epsilon \leq \frac{1}{2}+n\cdot \epsilon$ for all $j\in[m]$. Similarly, we can prove $\sum_j q'_{ij}\leq \frac{1}{2}+m\cdot \epsilon$ for all $i\in[n]$. As $\{\hat{q}_{ij}\}_{i\in[n],j\in[m]}$ is the optimal solution for the second convex program, $\sum_{i,j}R_{\hat{D}_{ij}}(\hat{q}_{ij})\geq \sum_{i,j}R_{\hat{D}_{ij}}({q}'_{ij})\geq \sum_{i,j}{R}_{D_{ij}}({q}^*_{ij})-\epsilon\cdot mn H$.
 \end{proof}

Finally, we show how to use the optimal solution of the convex program in Figure~\ref{fig:CP unit demand approximate dist} to construct an SPM that approximates the optimal revenue well. We first provide a general transformation that turns any approximately feasible solution of convex program in Figure~\ref{fig:CP unit demand} to an SPM mechanism.

\begin{lemma}\label{lem:prices to SPM}
	 For any distribution $\DD=\times_{i\in[n], j\in[m]}\DD_{ij}$, given a collection of independent random variables $\{p_{ij}\}_{i\in[n],j\in[m]}$ such that $$\sum_{i\in[n]} \Pr_{p_{ij}, t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\leq 1-\eta_1 \text{,\quad for all $j\in[m]$}$$ and $$\sum_{j\in[m]} \Pr_{p_{ij}, t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\leq 1-\eta_2 \text{,\quad for all $i\in[n]$},$$ we can construct in polynomial time a randomized SPM such that the revenue under $\DD$ is at least $$\eta_1 \eta_2\cdot \sum_{i, j} \E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\right].$$
	 \end{lemma}

\begin{proof}
	Consider a randomized SPM that sells item $j$ to bidder $i$ at price $p_{ij}$. Notice that bidder $i$ purchases exactly item $j$ if all of the following three conditions hold: (i) for all bidders $\ell\neq i$, $t_{\ell j}$ is smaller than the corresponding price $p_{\ell j}$,  (ii) for all items $k\neq j$, $t_{ik}$ is smaller than the corresponding price $p_{ik}$, and (iii) $t_{ij}$ is greater than the corresponding price $p_{ij}$. These three conditions are independent from each other. The first condition holds with probability at least $1-\sum_{\ell\neq i} \Pr_{p_{\ell j}, t_{\ell j}\sim \DD_{\ell j}}\left[t_{\ell j}\geq p_{\ell j}\right]\geq \eta_1$. The second condition holds with probability at least $1-\sum_{k \neq j} \Pr_{p_{ik}, t_{ik}\sim \DD_{ik}}\left[t_{ik}\geq p_{ik}\right]\geq \eta_2$. When the first two conditions hold, bidder $i$ purchases item $j$ whenever she can afford it. Her expected payment is $\E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\right]$. Hence, the expected revenue for selling item $j$ to bidder $i$ is at least $\eta_1\eta_2\cdot \E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\right]$ and the total expected revenue is at least $\eta_1 \eta_2\cdot \sum_{i, j} \E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim \DD_{ij}}\left[t_{ij}\geq p_{ij}\right]\right]$.
	
	\end{proof}

\begin{lemma}\label{lem:convert approx CP to SPM}
	Given any feasible solution $\{{q}_{ij}\}_{i\in[n],j\in[m]}$ of the convex program in Figure~\ref{fig:CP unit demand approximate dist}, we can construct a (randomized) SPM in polynomial time such that its revenue under $D$ is at least $\left(\frac{1}{4}-(n+m)\cdot \epsilon\right)\cdot \left( \sum_{i,j}R_{\hat{D}_{ij}}(q_{ij})-\epsilon\cdot nmH\right)$. 
\end{lemma}

\begin{proof}
	We first fix some notations. For any bidder $i$ and item $j$, let $\ubar{q}_{ij}, \bar{q}_{ij}$ and $x_{ij}$ $\in[0,1]$ be the numbers satisfying $x_{ij}\cdot \ubar{q}_{ij}\cdot \hat{F}_{ij}^{-1}(1-\ubar{q}_{ij}) +(1-x_{ij})\cdot \bar{q}_{ij}\cdot \hat{F}_{ij}^{-1}(1-\bar{q}_{ij})=R_{\hat{D}_{ij}}(q_{ij})$ and $x_{ij}\cdot \ubar{q}_{ij} +(1-x_{ij})\cdot \bar{q}_{ij}=q_{ij}$. We use $p_{ij}$ to denote a random variable that is $\ubar{p}_{ij} = \hat{F}_{ij}^{-1}(1-\ubar{q}_{ij})$ with probability $x_{ij}$ and $\bar{p}_{ij} = \hat{F}_{ij}^{-1}(1-\bar{q}_{ij})$ with probability $1-x_{ij}$.  
	
	Next, we construct a randomized SPM based on $\{p_{ij}\}_{i\in[n],j\in[m]}$ according to Lemma~\ref{lem:prices to SPM}. Note that $$\sum_{i\in[n]} \Pr_{p_{ij}, t_{ij}\sim D_{ij}}\left[t_{ij}\geq p_{ij}\right]\leq \sum_{i\in[n]} \left(\Pr_{p_{ij}, t_{ij}\sim \hat{D}_{ij}}\left[t_{ij}\geq p_{ij}\right]+\epsilon\right)=\sum_{i\in[n]} q_{ij}+n\epsilon\leq \frac{1}{2}+2n\epsilon$$ for all item $j$, and $$\sum_{j\in[m]} \Pr_{p_{ij}, t_{ij}\sim D_{ij}}\left[t_{ij}\geq p_{ij}\right]\leq \sum_{j\in[m]} \left(\Pr_{p_{ij}, t_{ij}\sim \hat{D}_{ij}}\left[t_{ij}\geq p_{ij}\right]+\epsilon\right)=\sum_{i\in[m]} q_{ij}+m\epsilon\leq \frac{1}{2}+2m\epsilon$$ for all bidder $i$. Hence, we can construct in polynomial time a randomized SPM with revenue at least \begin{align*} &\left(\frac{1}{2}-2n\epsilon\right)\left(\frac{1}{2}-2m\epsilon\right)\cdot \sum_{i, j} \E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim D_{ij}}\left[t_{ij}\geq p_{ij}\right]\right]\\
 	\geq &  \left(\frac{1}{4}-(n+m)\epsilon\right)\sum_{i, j} \E_{p_{ij}}\left[p_{ij}\cdot \left(\Pr_{t_{ij}\sim \hat{D}_{ij}}\left[t_{ij}\geq p_{ij}\right]-\epsilon\right)\right]\\
 	\geq & \left(\frac{1}{4}-(n+m)\epsilon\right)\sum_{i, j} \left(R_{\hat{D}_{ij}}(q_{ij})-\epsilon\cdot nmH\right)
 \end{align*}
	The first inequality is because $\left|\left|D_{ij}-\hat{D}_{ij}\right|\right|_K\leq \epsilon$, and the second inequality is because $p_{ij}$ is upper bounded by $H$ and $\E_{p_{ij}}\left[p_{ij}\cdot \Pr_{t_{ij}\sim \hat{D}_{ij}}\left[t_{ij}\geq p_{ij}\right]\right]=R_{\hat{D}_{ij}}(q_{ij})$ by the definition of $p_{ij}$.
	
	
	 %For bidder $i$, her price for item $j$ is $\ubar{p}_{ij}$ with probability $x_{ij}$ and $\bar{p}_{ij}$ with probability $1-x_{ij}$. This choice is made independently from all the other prices. The probability that bidder $i$ can afford this price is $q'_{ij}=x_{ij}\cdot\left(1-F_{ij}(\ubar{p}_{ij})\right)+(1-x_{ij})\cdot \left(1-F_{ij}(\bar{p}_{ij})\right)$. Since $||\hat{D}_{ij}-D_{ij}||_K\leq \epsilon$, $q'_{ij}\in [q_{ij}-\epsilon,q_{ij}+\epsilon]$. Notice that when it is buyer $i$'s turn, she purchases exactly item $j$ if all of the following three conditions hold: (i) for all bidders $\ell\neq i$, $t_{\ell j}$ is smaller than the corresponding price,  (ii) for all items $k\neq j$, $t_{ik}$ is smaller than the corresponding price, and (iii) $t_{ij}$ is greater than the corresponding price. All three conditions are independent from each other. The first condition holds with probability at least $1-\sum_{\ell\neq i} q'_{\ell j}\geq 1- \sum_{\ell\neq i} (q_{\ell j}+\epsilon)\geq \frac{1}{2}-2n\cdot \epsilon$. The second condition holds with probability at least $1-\sum_{k\neq j} q'_{ik}\leq 1-\sum_{k\neq j} (q_{ik}+\epsilon)\geq \frac{1}{2}-2m\cdot \epsilon$. When the two conditions hold, bidder $i$ buys item $j$ if she can afford it. The expected payment is 
\notshow{	 \begin{align*}
	&x_{ij}\cdot \ubar{p}_{ij}\cdot \left(1-F_{ij}(\ubar{p}_{ij})\right)+(1-x_{ij})\cdot\bar{p}_{ij}\cdot \left(1-F_{ij}(\bar{p}_{ij})\right)\\
	\geq &x_{ij}\cdot \ubar{p}_{ij}\cdot (\ubar{q}_{ij}-\epsilon)+(1-x_{ij})\cdot\bar{p}_{ij}\cdot (\bar{q}_{ij}-\epsilon)\geq R_{\hat{D}_{ij}}(q_{ij})-\epsilon\cdot H.\end{align*} 
	Therefore, the expected revenue of the randomized SPM is at least $$\left(\frac{1}{2}-2n\cdot \epsilon\right)\cdot \left(\frac{1}{2}-2m\cdot \epsilon\right)\cdot \left( \sum_{i,j}R_{\hat{D}_{ij}}(q_{ij})-\epsilon\cdot nmH\right)\geq \left(\frac{1}{4}-(n+m)\cdot \epsilon\right)\cdot \left( \sum_{i,j}R_{\hat{D}_{ij}}(q_{ij})-\epsilon\cdot nmH\right).$$} 
	\end{proof}


\begin{theorem}\label{thm:UD Kolmogorov}
For unit-demand bidders, given distributions $\hat{D}_{ij}$ where $\left|\left|\hat{D}_{ij}-D_{ij}\right|\right|_K\leq \epsilon$ for all $i\in[n]$ and $j\in[m]$, there is a polynomial time algorithm that constructs a randomized SPM whose revenue under $D$ is at least $\left(\frac{1}{4}-(n+m)\cdot \epsilon\right)\cdot\left(\frac{\opt}{8}-2\epsilon\cdot mnH\right)$.
\end{theorem}

\begin{proof}
	Our algorithm first computes the optimal solution $\{\hat{q}_{ij}\}_{i\in[n],j\in[m]}$ for the convex program in Figure~\ref{fig:CP unit demand approximate dist}, then  constructs a randomized SPM based on $\{\hat{q}_{ij}\}_{i\in[n],j\in[m]}$ using Lemma~\ref{lem:convert approx CP to SPM}. It is not hard to see that our algorithm runs in polynomial time. By chaining the inequalities in Lemma~\ref{lem:compare exact CP with opt},~\ref{lem:UD compare the two CP} and~\ref{lem:convert approx CP to SPM}, we can argue that the revenue of our mechanism is at least $\left(\frac{1}{4}-(n+m)\cdot \epsilon\right)\cdot\left(\frac{\opt}{8}-2\epsilon\cdot mnH\right)$.
\end{proof}

\subsection{Unit-demand Valuation: sample access to bounded distributions} 

When the distributions $D_{ij}$ are all bounded, the following theorem provides the sample complexity.
\begin{theorem}\cite{MorgensternR16}\label{thm:UD bounded}
	When $D_{ij}$ is supported on $[0,H]$ for all bidder $i$ and item $j$, the sample complexity for $(\epsilon,\delta)$-uniformly learning the revenue of SPMs for unit-demand bidders is $O\left(\left(\frac{1}{\epsilon}\right)^2 \left(m^2 n\log n\log \frac{1}{\epsilon} + \log \frac{1}{\delta}\right)\right)$. That is, with probability $1-\delta$, the empirical revenue based on the samples for any SPM is within $\epsilon\cdot H$ of its true expected revenue. %samples suffices to learn with probability $1-\delta$ an SPM whose revenue is at most $\epsilon H$ less than the best SPM whose revenue is at least $\frac{\opt}{24}$. 
	\yangnote{Moreover, with the same number of samples, there is a polynomial time algorithm that learns an SPM whose revenue is at least $\frac{\opt}{144}-\epsilon H$ with probability $1-\delta$. } \cnote{Shouldn't there be a $(H/\epsilon)^2$ in the sample complexity??}\end{theorem}


\subsection{Unit-demand Valuation: sample access to regular distributions}
In this section, we show there exists a polynomial time algorithm that learns an SPM whose revenue is at least a constant fraction of the optimal revenue with polynomial in $n$ and $m$ samples. Note that unlike in the previous two models, the error of our learning algorithm is only multiplicative when the distributions are regular. First, we present a Lemma regarding the revenue curve function for regular distributions.


%                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               Let us first sketch the proof. First, we use the property that all distributions are regular to argue that restricting the posted prices to be less than some upper bound $H= O\left(\poly(n,m)\cdot \opt\right)$ will affect the best revenue achievable by an SPM by at most a small multiplicative factor. In the second step, we truncate the original distributions $D_{ij}$ at the upper bound $H$ and argue that the revenue for any SPM under $D$ and the truncated distribution are exactly the same. Next, we apply Theorem~\ref{thm:UD bounded} to the truncated distribution to obtain an SPM. The only issue here is that Theorem~\ref{thm:UD bounded} has an additive error that depends on $H$. Luckily, since $H$ is at most a polynomial times larger than $\opt$ we can simply choose $\epsilon$ to be inverse of some polynomial to convert the additive error of $\epsilon H$ into a multiplicative error.

\begin{lemma}\cite{CaiD11b}\label{lem:regular revenue curve concave}
	For any regular distribution $F$, let $R_F(\cdot)$ be the corresponding revenue curve. For any $0<q'\leq q\leq  p < 1$, $$(1-p)\cdot R_F(q')\leq  R_F(q).$$
	\end{lemma}
 Throughout this section, we use $Z$ to denote $\max\{m,n\}$ and $C$ to be a constant that will be specified later. Using Lemma~\ref{lem:regular revenue curve concave}, we show in the next Lemma that restricting $q_{ij}$ to be at least $\frac{1}{ CZ}$ does not affect the objective value of the convex program in Figure~\ref{fig:CP unit demand} by too much.

\begin{lemma}\label{lem:lowering high prices}
	Suppose $\{q_{ij}^*\}_{i\in[n], j\in[m]}$ is the optimal solution of the convex program in Figure~\ref{fig:CP unit demand}. Let $q'_{ij}=\max\{\frac{1}{CZ}, q^*_{ij}\}$, then $\sum_{i,j} R_{D_{ij}}(q'_{ij})\geq \left(1-\frac{1}{ CZ}\right)\cdot \sum_{i,j} R_{D_{ij}}(q^*_{ij})\geq \left(1-\frac{1}{ CZ}\right)\cdot \frac{\opt}{8}$.
\end{lemma}
\begin{proof}
	According to Lemma~\ref{lem:compare exact CP with opt}, $\sum_{i,j} R_{D_{ij}}(q^*_{ij})\geq \frac{\opt}{8}$. So to prove the statement, it suffices to argue that for any $i$ and $j$, $R_{D_{ij}}(q'_{ij})\geq \left(1-\frac{1}{CZ}\right)\cdot R_{D_{ij}}(q^*_{ij})$. If $q^*_{ij} = q'_{ij}$, this inequality clearly holds. If $q^*_{ij} \neq q'_{ij}$, $q^*_{ij}\leq q'_{ij}=\frac{1}{CZ}$. Since $F_{ij}$ is regular, we can apply Lemma~\ref{lem:regular revenue curve concave} to $q'_{ij}$ and $q^*_{ij}$ and obtain inequality $R_{D_{ij}}(q'_{ij})\geq \left(1-\frac{1}{C Z}\right)\cdot R_{D_{ij}}(q^*_{ij})$.
\end{proof}

Using Lemma~\ref{lem:lowering high prices}, we argue how to compute in polynomial time an approximately optimal SPM. Suppose $D'_{ij}$ is the distribution that we obtain after truncating $D_{ij}$ at a threshold $H_{ij}$\footnote{Let $t_{ij}\sim D_{ij}$, then $\min\{t_{ij},H_{ij}\}$ is the corresponding truncated random variable drawn from $D'_{ij}$.}, and we have direct access to a discrete distribution $\hat{D}'_{ij}$ such that $\left|\left|\hat{D}'_{ij}-D'_{ij}\right|\right|_K\leq \epsilon$ for all $i$ and $j$. We show in the following Lemma that the optimal solution of a convex program similar to the one in Figure~\ref{fig:CP unit demand approximate dist} but for $\{\hat{D}'_{ij}\}_{i\in[n],j\in[m]}$ can guide us to design an approximately optimal SPM under $D$ in polynomial time. As we have sample access to $D$, we will argue later that a polynomial number of samples suffices to generate $\{\hat{D}'_{ij}\}_{i\in[n],j\in[m]}$.%Then for any SPM that does not use price $p_{ij}> H_{ij}$, its revenue under $D'=\times_{i,j} D'_{ij}$ and $D$ is the same. Therefore, if we can learn an SPM with good revenue for $D'$, the same mechanism also achieves good revenue under $D$.
\notshow{\begin{lemma}\label{lem:UD low prices suffice}
	There exists a collection of deterministic prices $\{p'_{ij}\}_{i\in[n],j\in[m]}$ satisfying $F_{ij}(p'_{ij})\leq 1-\frac{1}{C\cdot Z}$ for all $i\in[n]$ and $j\in[m]$, such that the corresponding SPM achieves revenue of $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}$.
\end{lemma} 
\begin{proof}
Let $\{q_{ij}^*\}_{i\in[n], j\in[m]}$ be the optimal solution of the convex program in Figure~\ref{fig:CP unit demand} and $q'_{ij}=\max\{\frac{1}{C\cdot Z}, q^*_{ij}\}$. For every $i$ and $j$, let $p'_{ij}$ to be $F^{-1}_{ij}(1-q'_{ij})$. Clearly, $F_{ij}(p'_{ij})\leq 1-\frac{1}{C\cdot Z}$. 

As $D_{ij}$ is regular, $R_{D_{ij}}(q'_{ij}) = p'_{ij} q'_{ij}$. Therefore, $\sum_{i,j} p'_{ij}q'_{ij}=\sum_{i,j} R_{D_{ij}}(q'_{ij})\geq \left(1-\frac{1}{CZ} \right)\cdot \frac{\opt}{8}$ according to Lemma~\ref{lem:UD low prices suffice}. Also, $\sum_i q'_{ij}\leq \frac{1}{2}+\frac{n}{CZ}\leq \frac{1}{2}+\frac{1}{C}$ for all item $j$, and $\sum_j q'_{ij}\leq \frac{1}{2}+\frac{m}{CZ}\leq \frac{1}{2}+\frac{1}{C}$ for all bidder $i$. According to Lemma~\ref{lem:prices to SPM}, the SPM with prices $\{p'_{ij}\}_{i\in[n],j\in[m]}$ has revenue at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \sum_{i,j} p'_{ij}q'_{ij}\geq \left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot  \left(1-\frac{1}{CZ} \right)\cdot \frac{\opt}{8}$.

%Next, we argue that if we use $p_{ij}$ as the prices in an SPM, the expected revenue is at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}$. For any $i$ and $j$, the probability that (i) all bidders $\ell\neq i$ cannot afford item $j$ and (ii) bidder $i$ cannot afford the price for any item $k\neq j$ is at least $\left(1-\sum_{\ell\neq i}q'_{\ell j}\right)\cdot \left(1-\sum_{k\neq j}q'_{ik}\right)$. Since both $\sum_\ell q^*_{\ell j}$ and $\sum_{k}q^*_{ik}$ are less than $\frac{1}{2}$, both $1-\sum_{\ell\neq i}q'_{\ell j}$ and $1-\sum_{k\neq j}q'_{ik}$ are at least $\frac{1}{2}-\frac{1}{C}$. Clearly, when (i) and (ii) are simultaneously satisfied, bidder $i$ purchases item $j$ whenever $t_{ij}$ is greater than $p_{ij}$. Therefore, the total revenue of this SPM is at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \sum_{i,j} p_{ij}\cdot q'_{ij}$. As $F_{ij}$ is regular, $p_{ij}\cdot q'_{ij}=R_{D_{ij}}(q'_{ij})$. Finally, we know that  $\sum_{i,j} R_{D_{ij}}(q'_{ij})\geq \left(1-\frac{1}{C\cdot Z}\right)\cdot \sum_{i,j} R_{D_{ij}}(q^*_{ij})\geq \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}$ from Lemma~\ref{lem:lowering high prices} and~\ref{lem:compare exact CP with opt}. Combining this inequality with the lower bound of the revenue for the SPM, we can show that the revenue of our constructed SPM is at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}$.
\end{proof}



\begin{lemma}\label{lem:UD additive bound}
	Let $\{H_{ij}\}_{i\in[n],j\in[m]}$ be a collection of positive numbers satisfying $F_{ij}(H_{ij})\in [1-\frac{1}{C\cdot Z}, 1-\frac{1}{3C\cdot Z}]$ for all $i\in[n]$ and $j\in[m]$. With $O\left(\left(\frac{1}{\epsilon}\right)^2 \left(m^2 n\log n\log \frac{1}{\epsilon} + \log \frac{1}{\delta}\right)\right)$ samples, we can learn an SPM with probability $1-\delta$ that achieves revenue at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}-\epsilon\cdot\max_{i,j} H_{ij}$. \yangnote{With the same number of samples, we can learn in polynomial time an SPM with probability $1-\delta$ that achieves revenue at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{48}-\epsilon\cdot\max_{i,j} H_{ij}$.}
\end{lemma}
\begin{proof}
	First, we truncate each $D_{ij}$ at $H_{ij}$ to create a bounded distribution $D'_{ij}$. This is straightforward, as we only need to cap the value for any sample from $D_{ij}$ at $H_{ij}$. According to Lemma~\ref{lem:UD low prices suffice}, there exists an SPM that achieves revenue at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}$ under $D'=\times_{i,j} D'_{ij}$, as the price $p_{ij}$ used in the SPM is less than $H_{ij}$ for all $i,j$. Combining this observation with Theorem~\ref{thm:UD bounded}, we know that if we take $O\left(\left(\frac{1}{\epsilon}\right)^2 \left(m^2 n\log n\log \frac{1}{\epsilon} + \log \frac{1}{\delta}\right)\right)$ samples we can learn with probability $1-\delta$ an SPM whose revenue is at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}-\epsilon\cdot\max_{i,j} H_{ij}$. Similarly, we can prove the computational friendly version of this claim. \end{proof}}
	
\begin{lemma}\label{lem:UD additive bound}
	Let $\{H_{ij}\}_{i\in[n],j\in[m]}$ be a collection of positive numbers satisfying $F_{ij}(H_{ij})\in [1-\frac{1}{C\cdot Z}, 1-\frac{1}{3C\cdot Z}]$ for all $i\in[n]$ and $j\in[m]$. Let $D'_{ij}$ be the distribution of the random variable $\min\{t_{ij}, H_{ij}\}$ where $t_{ij}\sim D_{ij}$, and $\hat{D}_{ij}'$ be a discrete distribution such that $\left|\left|\hat{D}'_{ij}-D'_{ij}\right|\right|_K\leq \epsilon$ for all $i\in[n]$ and $j\in[m]$. Suppose $s$ is an upper bound of the support size for any distribution $\hat{D}'_{ij}$, then given direct access to $\hat{D}_{ij}'$, we can compute in time polynomial in $n$, $m$ and $s$ a randomized SPM that achieves revenue at least $\left(\frac{1}{2}-\frac{1}{C}-2n\epsilon\right)\cdot\left(\frac{1}{2}-\frac{1}{C}-2m\epsilon\right)\cdot \left(\left(1-\frac{1}{ CZ}\right)\cdot \frac{\opt}{8}-2\epsilon\cdot nmH\right)$ under $D$, where $H= \max_{i,j} H_{ij}$. 
\end{lemma}
\begin{proof}
Consider the following convex program:

\begin{minipage}{\textwidth} 
\begin{align*}
&\max \sum_{i,j} R_{\hat{D}_{ij}'}(q_{ij})\\
\textbf{s.t. }& \sum_i q_{ij}\leq \frac{1}{2} + \frac{1}{C} +n\cdot\epsilon\qquad \text{ for all $j\in[m]$}\\
& \sum_j q_{ij}\leq \frac{1}{2}+\frac{1}{C} +m\cdot\epsilon \qquad \text{ for all $i\in[n]$}\\
& q_{ij}\geq 0\qquad \text{ for all $i\in[n]$ and $j\in[m]$}
\end{align*}
\end{minipage}
\vspace{.1in}

Let $\{q_{ij}^*\}_{i\in[n], j\in[m]}$ be the optimal solution of the convex program in Figure~\ref{fig:CP unit demand} and $q'_{ij}=\max\{\frac{1}{C\cdot Z}, q^*_{ij}\}$. For every $i$ and $j$, let $p'_{ij}=F^{-1}_{ij}(1-q'_{ij})$ and $\tilde{q}_{ij} = \Pr_{t_{ij}\sim \hat{D}'_{ij}}\left[t_{ij}\geq p'_{ij}\right]$. By the definition of $H_{ij}$, $p'_{ij}\leq H_{ij}$, so \begin{align}\label{ineq:LB inequality}
p'_{ij}\tilde{q}_{ij}\geq p'_{ij}\left(\Pr_{t_{ij}\sim {D}'_{ij}}\left[t_{ij}\geq p'_{ij}\right]-\epsilon\right)\geq p'_{ij} q'_{ij}-\epsilon\cdot H_{ij}=R_{D_{ij}}(q'_{ij})-\epsilon\cdot H_{ij}.
 \end{align}
$p'_{ij} q'_{ij}$ equals to $R_{D_{ij}}(q'_{ij})$ because $D_{ij}$ is a regular distribution.

Next, we argue that $\{\tilde{q}_{ij}\}_{i\in[n],j\in[m]}$ is a feasible solution of the convex program above. Observe that $$\sum_{i} \tilde{q}_{ij} \leq \sum_i q'_{ij}+n\epsilon \leq \sum_i \left(q^*_{ij}+\frac{1}{CZ}\right)+n\epsilon\leq \frac{1}{2} + \frac{1}{C} +n\epsilon$$ for all item $j\in[m]$ and $$\sum_{j} \tilde{q}_{ij} \leq \sum_j q'_{ij}+n\epsilon \leq \sum_j \left(q^*_{ij}+\frac{1}{CZ}\right)+m\epsilon\leq \frac{1}{2}+\frac{1}{C} +m\epsilon$$ for all bidder $i\in[n]$. 

 Let $\widehat{\opt}$ be the optimal solution of the convex program above. As $\{\tilde{q}_{ij}\}_{i\in[n],j\in[m]}$ is a feasible solution,
$$\widehat{\opt}\geq \sum_{i,j} R_{\hat{D}_{ij}'}(\tilde{q}_{ij})\geq \sum_{i,j} p'_{ij}\tilde{q}_{ij}\geq \sum_{i,j} R_{D_{ij}}(q'_{ij})-\epsilon\cdot nmH\geq \left(1-\frac{1}{ CZ}\right)\cdot \frac{\opt}{8}-\epsilon\cdot nmH.$$
The second last inequality is due to inequality~(\ref{ineq:LB inequality}) and the last inequality is due to Lemma~\ref{lem:lowering high prices}.

So far, we have argued that the optimal solution of our convex program has value close to the $\opt$. We will show in the second part of the proof that using the optimal solution of our convex program, we can construct an SPM whose revenue under $D$ is close to $\widehat{\opt}$. Let $\hat{q}_{ij}$ be the optimal solution of the convex program above and $\hat{p}_{ij}$ be the corresponding random price, that is, $\Pr_{\hat{p}_{ij}, t_{ij}\sim \hat{D}_{ij}'}\left[t_{ij}\geq \hat{p}_{ij}\right]=\hat{q}_{ij}$ and $R_{\hat{D}_{ij}'}(\hat{q}_{ij}) = \E_{\hat{p}_{ij}}\left[\hat{p}_{ij}\cdot \Pr_{t_{ij}\sim \hat{D}_{ij}'}\left[t_{ij}\geq \hat{p}_{ij}\right]\right]$. As $\hat{p}_{ij}\leq H_{ij}$, $$\Pr_{\hat{p}_{ij}, t_{ij}\sim {D}_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]=\Pr_{\hat{p}_{ij}, t_{ij}\sim {D}'_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]\in  [\hat{q}_{ij}-\epsilon,\hat{q}_{ij}+\epsilon].$$ Therefore, for all item $j$ $$\sum_{i} \Pr_{\hat{p}_{ij}, t_{ij}\sim {D}_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]\leq \sum_{i} \Pr_{\hat{p}_{ij}, t_{ij}\sim \hat{D}_{ij}'}\left[t_{ij}\geq \hat{p}_{ij}\right] + n\epsilon = \sum_i \hat{q}_{ij} +n\epsilon \leq \frac{1}{2} + \frac{1}{C} +2n\epsilon$$ and for all bidder $i$	$$\sum_{j} \Pr_{\hat{p}_{ij}, t_{ij}\sim {D}_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]\leq \sum_{j} \Pr_{\hat{p}_{ij}, t_{ij}\sim \hat{D}_{ij}'}\left[t_{ij}\geq \hat{p}_{ij}\right] + m\epsilon = \sum_j \hat{q}_{ij} +m\epsilon \leq \frac{1}{2} + \frac{1}{C} +2m\epsilon.$$ According to Lemma~\ref{lem:prices to SPM}, we can construct a randomized SPM with $\{\hat{p}_{ij}\}_{i\in[n],j\in[m]}$ whose revenue is at least $\left(\frac{1}{2}-\frac{1}{C}-2n\epsilon\right)\cdot\left(\frac{1}{2}-\frac{1}{C}-2m\epsilon\right)\cdot \sum_{i,j} \E_{\hat{p}_{ij}}\left[\hat{p}_{ij}\cdot \Pr_{t_{ij}\sim {D}_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]\right]$ under $D$. 
Clearly, $$\E_{\hat{p}_{ij}}\left[\hat{p}_{ij}\cdot \Pr_{t_{ij}\sim {D}_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]\right]\geq \E_{\hat{p}_{ij}}\left[\hat{p}_{ij}\cdot \left(\Pr_{t_{ij}\sim \hat{D}'_{ij}}\left[t_{ij}\geq \hat{p}_{ij}\right]-\epsilon\right)\right] = R_{\hat{D}'_{ij}}(\hat{q}_{ij})-\epsilon\cdot H_{ij}.$$ Therefore, the revenue of the constructed randomized SPM under $D$ is at least \begin{align*} &\left(\frac{1}{2}-\frac{1}{C}-2n\epsilon\right)\cdot\left(\frac{1}{2}-\frac{1}{C}-2m\epsilon\right)\cdot \left(\widehat{\opt}-\epsilon\cdot nmH\right)\\
 	\geq & \left(\frac{1}{2}-\frac{1}{C}-2n\epsilon\right)\cdot\left(\frac{1}{2}-\frac{1}{C}-2m\epsilon\right)\cdot \left(\left(1-\frac{1}{ CZ}\right)\cdot \frac{\opt}{8}-2\epsilon\cdot nmH\right).
 \end{align*}
It is not hard to see that both $\{\hat{q}_{ij}\}_{i\in[n],j\in[m]}$ and $\{\hat{p}_{ij}\}_{i\in[n],j\in[m]}$ can be computed in time polynomial in $n$, $m$ and $s$.
	\end{proof}

	When $\epsilon$ is small enough, we can turn the additive error in Lemma~\ref{lem:UD additive bound} into a multiplicative error. Next, we argue that with a polynomial number of samples, we can learn $\{H_{ij}\}_{i\in[n],j\in[m]}$ and $\{\hat{D}'_{ij}\}_{i\in[n],j\in[m]}$ with enough accuracy.

\begin{theorem}\label{thm:UD regular}
If for all bidder $i$ and item $j$, $D_{ij}$ is a regular distribution, we can learn in polynomial time with probability $1-\delta$ a randomized SPM whose revenue is at least $\frac{\opt}{33}$ with $O\left(Z^2m^2 n^2\cdot \left(\log n +\log m + \log \frac{1}{\delta}\right)\right)$ ($Z=\max\{m,n\}$) samples. %\yangnote{With the same number of samples, we can learn in polynomial time with probability $1-\delta$ an SPM whose revenue is at least $\frac{\opt}{198}$.}
\end{theorem}
\begin{proof}
	First, if we take $O\left(C^2\cdot Z^2\cdot \left(\log (nm)+\log \frac{1}{\delta}\right)\right)$ samples from each $D_{ij}$, we can estimate $H_{ij}$ such that $F_{ij}(H_{ij})\in[1-\frac{1}{C\cdot Z}, 1-\frac{1}{3C\cdot Z}]$ with probability $1-\frac{\delta}{2nm}$. By the union bound, the probability that all $H_{ij}$ satisfy the requirement is at least $1-\frac{\delta}{2}$. From now on, we only consider the case where $H_{ij}$ satisfies $F_{ij}(H_{ij})\in[1-\frac{1}{C\cdot Z}, 1-\frac{1}{3C\cdot Z}]$ for all $i$ and $j$. Next, we observe that $\opt \geq \max_{i,j} H_{ij}\cdot \frac{1}{3C\cdot Z}$, as the expected revenue for selling item $j$ to bidder $i$ with price $H_{ij}$ is at least $ \frac{H_{ij}}{3C\cdot Z}$. Therefore, there exists sufficiently large constant $d$ and $C$, if $\epsilon=\frac{1}{d\cdot Z nm}$ the randomized SPM learned in Lemma~\ref{lem:UD additive bound} has revenue at least $\frac{\opt}{33}$. According to the Dvoretzky-Kiefer-Wolfowitz (DKW) inequality~\cite{DvoretzkyKW56}, if we take $O\left(d^2 Z^2n^2m^2\cdot \left(\log \frac{1}{\delta}+\log n+\log m\right) \right)$ i.i.d. samples from $D'_{ij}$ (we can take samples from $D_{ij}$ then cap the samples at $H_{ij}$) and let $\hat{D}'_{ij}$ be the empirical distribution induced by the samples, $\left|\left|D'_{ij}-\hat{D}'_{ij}\right|\right|_K\leq \frac{1}{d\cdot Z nm}$ with probability $1-\frac{\delta}{2nm}$. By the union bound, $\left|\left|D'_{ij}-\hat{D}'_{ij}\right|\right|_K\leq \frac{1}{d\cdot Z nm}$ for all $i\in[n]$ and $j\in[m]$ with probability at least $1-\delta/2$. Finally, if we take another union bound over the choice of $\{H_{ij}\}_{i\in[n],j\in[m]}$ and $\{\hat{D}'_{ij}\}_{i\in[n],j\in[m]}$, we can learn a randomized SPM with probability at least $1-\delta$ using $O\left( Z^2n^2m^2\cdot \left(\log \frac{1}{\delta}+\log n+\log m\right) \right)$ samples. Furthermore, the support size of any $\hat{D}'_{ij}$ is at most $O\left( Z^2n^2m^2\cdot \left(\log \frac{1}{\delta}+\log n+\log m\right) \right)$, so our learning algorithm runs in time polynomial in $n$ and $m$.
	
	%To turn the additive error in Lemma~\ref{lem:UD additive bound} into a multiplicative error, $\epsilon$ needs to be as small as  Hence, we can learn with probability $1-\frac{\delta}{2}$ an SPM whose revenue is at least $\left(\frac{1}{2}-\frac{1}{C}\right)^2\cdot \left(1-\frac{1}{C\cdot Z}\right)\cdot \frac{\opt}{8}-3C Z\cdot\opt\cdot  \epsilon$, if we are given $O\left(\left(\frac{1}{\epsilon}\right)^2 \left(m^2 n\log n\log \frac{1}{\epsilon} + \log \frac{1}{\delta}\right)\right)$ samples. We let $\epsilon$ to be $\frac{1}{C^2\cdot Z}$. If $C$ is sufficiently big, the SPM learnt has revenue at least $\frac{\opt}{33}$  with probability $1-\frac{\delta}{2}$ and the number of samples needed is $O\left(Z^2 \cdot\left(m^2 n\log n\log Z + \log \frac{1}{\delta}\right)\right)$. 
	
	%To sum up, with $$O\left(Z^2 \cdot\left(m^2 n\log n\log Z + \log \frac{1}{\delta}\right)\right)+O\left(Z^2\cdot \left(\log (nm)+\log \frac{1}{\delta}\right)\right)= O\left(Z^2 \cdot\left(m^2 n\log n\log Z + \log \frac{1}{\delta}\right)\right)$$ samples we can learn an SPM whose revenue is at least $\frac{\opt}{33}$ with probability $1-\delta$. Similarly, we can prove the computational friendly version of this claim.
\end{proof}






